A Deep Neural Network for Pixel-Level Electromagnetic Particle Identification in the MicroBooNE Liquid Argon Time Projection Chamber

We have developed a convolutional neural network (CNN) that can make a pixel-level prediction of objects in image data recorded by a liquid argon time projection chamber (LArTPC) for the first time. We describe the network design, training techniques, and software tools developed to train this network. The goal of this work is to develop a complete deep neural network based data reconstruction chain for the MicroBooNE detector. We show the first demonstration of a network's validity on real LArTPC data using MicroBooNE collection plane images. The demonstration is performed for stopping muon and a $\nu_\mu$ charged current neutral pion data samples.

==> authors.tex <==
\newcommand{\Bern}{Universit{\"a}t Bern, Bern CH-3012, Switzerland}
\newcommand{\BNL}{Brookhaven National Laboratory (BNL), Upton, NY, 11973, USA}
\newcommand{\Cambridge}{University of Cambridge, Cambridge CB3 0HE, United Kingdom}
\newcommand{\Chicago}{University of Chicago, Chicago, IL, 60637, USA}
\newcommand{\Cincinnati}{University of Cincinnati, Cincinnati, OH, 45221, USA}
\newcommand{\CSU}{Colorado State University, Fort Collins, CO, 80523, USA}
\newcommand{\Columbia}{Columbia University, New York, NY, 10027, USA}
\newcommand{\FNAL}{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}
\newcommand{\Harvard}{Harvard University, Cambridge, MA 02138, USA}
\newcommand{\IIT}{Illinois Institute of Technology (IIT), Chicago, IL 60616, USA}
\newcommand{\KSU}{Kansas State University (KSU), Manhattan, KS, 66506, USA}
\newcommand{\Lancaster}{Lancaster University, Lancaster LA1 4YW, United Kingdom}
\newcommand{\LANL}{Los Alamos National Laboratory (LANL), Los Alamos, NM, 87545, USA}
\newcommand{\Manchester}{The University of Manchester, Manchester M13 9PL, United Kingdom}
\newcommand{\MIT}{Massachusetts Institute of Technology (MIT), Cambridge, MA, 02139, USA}
\newcommand{\Michigan}{University of Michigan, Ann Arbor, MI, 48109, USA}
\newcommand{\NMSU}{New Mexico State University (NMSU), Las Cruces, NM, 88003, USA}
\newcommand{\Otterbein}{Otterbein University, Westerville, OH, 43081, USA}
\newcommand{\Oxford}{University of Oxford, Oxford OX1 3RH, United Kingdom}
\newcommand{\PNNL}{Pacific Northwest National Laboratory (PNNL), Richland, WA, 99352, USA}
\newcommand{\Pitt}{University of Pittsburgh, Pittsburgh, PA, 15260, USA}
\newcommand{\StMarys}{Saint Mary's University of Minnesota, Winona, MN, 55987, USA}
\newcommand{\SLAC}{SLAC National Accelerator Laboratory, Menlo Park, CA, 94025, USA}
\newcommand{\Syracuse}{Syracuse University, Syracuse, NY, 13244, USA}
\newcommand{\TelAviv}{Tel Aviv University, Tel Aviv, Israel, 69978}
\newcommand{\Tennessee}{University of Tennessee, Knoxville, TN, 37996, USA}
\newcommand{\UTA}{University of Texas, Arlington, TX, 76019, USA}
\newcommand{\Tubitak}{TUBITAK Space Technologies Research Institute, METU Campus, TR-06800, Ankara, Turkey}
\newcommand{\Tufts}{Tufts University, Medford, MA, 02155, USA}
\newcommand{\VTech}{Center for Neutrino Physics, Virginia Tech, Blacksburg, VA, 24061, USA}
\newcommand{\Yale}{Yale University, New Haven, CT, 06520, USA}

% So that institutions appear in alphabetical order:
\affiliation{\Bern}
\affiliation{\BNL}
\affiliation{\Cambridge}
\affiliation{\Chicago}
\affiliation{\Cincinnati}
\affiliation{\CSU}
\affiliation{\Columbia}
\affiliation{\FNAL}
\affiliation{\Harvard}
\affiliation{\IIT}
\affiliation{\KSU}
\affiliation{\Lancaster}
\affiliation{\LANL}
\affiliation{\Manchester}
\affiliation{\MIT}
\affiliation{\Michigan}
\affiliation{\NMSU}
\affiliation{\Otterbein}
\affiliation{\Oxford}
\affiliation{\PNNL}
\affiliation{\Pitt}
\affiliation{\StMarys}
\affiliation{\SLAC}
\affiliation{\Syracuse}
\affiliation{\TelAviv}
\affiliation{\Tennessee}
\affiliation{\UTA}
\affiliation{\Tubitak}
\affiliation{\Tufts}
\affiliation{\VTech}
\affiliation{\Yale}

% Authors in alphabetical order
\author{C.~Adams} \affiliation{\Yale}
\author{M.~Alrashed} \affiliation{\KSU}
\author{R.~An} \affiliation{\IIT}
\author{J.~Anthony} \affiliation{\Cambridge}
\author{J.~Asaadi} \affiliation{\UTA}
\author{A.~Ashkenazi} \affiliation{\MIT}
\author{M.~Auger} \affiliation{\Bern}
\author{S.~Balasubramanian} \affiliation{\Yale}
\author{B.~Baller} \affiliation{\FNAL}
\author{C.~Barnes} \affiliation{\Michigan}
\author{G.~Barr} \affiliation{\Oxford}
\author{M.~Bass} \affiliation{\BNL}
\author{F.~Bay} \affiliation{\Tubitak}
\author{A.~Bhat} \affiliation{\Syracuse}
\author{K.~Bhattacharya} \affiliation{\PNNL}
\author{M.~Bishai} \affiliation{\BNL}
\author{A.~Blake} \affiliation{\Lancaster}
\author{T.~Bolton} \affiliation{\KSU}
\author{L.~Camilleri} \affiliation{\Columbia}
\author{D.~Caratelli} \affiliation{\Columbia}\affiliation{\FNAL}
\author{I.~Caro Terrazas} \affiliation{\CSU}
\author{R.~Carr} \affiliation{\MIT}
\author{R.~Castillo~Fernandez} \affiliation{\FNAL}
\author{F.~Cavanna} \affiliation{\FNAL}
\author{G.~Cerati} \affiliation{\FNAL}
\author{Y.~Chen} \affiliation{\Bern}
\author{E.~Church} \affiliation{\PNNL}
\author{D.~Cianci} \affiliation{\Columbia}
\author{E.~Cohen} \affiliation{\TelAviv}
\author{G.~H.~Collin} \affiliation{\MIT}
\author{J.~M.~Conrad} \affiliation{\MIT}
\author{M.~Convery} \affiliation{\SLAC}
\author{L.~Cooper-Troendle} \affiliation{\Yale}
\author{J.~I.~Crespo-Anad\'{o}n} \affiliation{\Columbia}
\author{M.~Del~Tutto} \affiliation{\Oxford}
\author{D.~Devitt} \affiliation{\Lancaster}
\author{A.~Diaz} \affiliation{\MIT}
\author{K. Duffy} \affiliation{\FNAL}
\author{S.~Dytman} \affiliation{\Pitt}
\author{B.~Eberly} \affiliation{\SLAC}
\author{A.~Ereditato} \affiliation{\Bern}
\author{L.~Escudero Sanchez} \affiliation{\Cambridge}
\author{J.~Esquivel} \affiliation{\Syracuse}
\author{J.~J~Evans} \affiliation{\Manchester}
\author{A.~A.~Fadeeva} \affiliation{\Columbia}
\author{R.~S.~Fitzpatrick} \affiliation{\Michigan}
\author{B.~T.~Fleming} \affiliation{\Yale}
\author{D.~Franco} \affiliation{\Yale}
\author{A.~P.~Furmanski} \affiliation{\Manchester}
\author{D.~Garcia-Gamez} \affiliation{\Manchester}
\author{G.~T.~Garvey} \affiliation{\LANL}
\author{V.~Genty} \affiliation{\Columbia}
\author{D.~Goeldi} \affiliation{\Bern}
\author{S.~Gollapinni} \affiliation{\Tennessee}
\author{O.~Goodwin} \affiliation{\Manchester}
\author{E.~Gramellini} \affiliation{\Yale}
\author{H.~Greenlee} \affiliation{\FNAL}
\author{R.~Grosso} \affiliation{\Cincinnati}
\author{R.~Guenette} \affiliation{\Harvard}
\author{P.~Guzowski} \affiliation{\Manchester}
\author{A.~Hackenburg} \affiliation{\Yale}
\author{P.~Hamilton} \affiliation{\Syracuse}
\author{O.~Hen} \affiliation{\MIT}
\author{J.~Hewes} \affiliation{\Manchester}
\author{C.~Hill} \affiliation{\Manchester}
\author{G.~A.~Horton-Smith} \affiliation{\KSU}
\author{A.~Hourlier} \affiliation{\MIT}
\author{E.-C.~Huang} \affiliation{\LANL}
\author{C.~James} \affiliation{\FNAL}
\author{J.~Jan~de~Vries} \affiliation{\Cambridge}
\author{L.~Jiang} \affiliation{\Pitt}
\author{R.~A.~Johnson} \affiliation{\Cincinnati}
\author{J.~Joshi} \affiliation{\BNL}
\author{H.~Jostlein} \affiliation{\FNAL}
\author{Y.-J.~Jwa} \affiliation{\Columbia}
\author{G.~Karagiorgi} \affiliation{\Columbia}
\author{W.~Ketchum} \affiliation{\FNAL}
\author{B.~Kirby} \affiliation{\BNL}
\author{M.~Kirby} \affiliation{\FNAL}
\author{T.~Kobilarcik} \affiliation{\FNAL}
\author{I.~Kreslo} \affiliation{\Bern}
\author{Y.~Li} \affiliation{\BNL}
\author{A.~Lister} \affiliation{\Lancaster}
\author{B.~R.~Littlejohn} \affiliation{\IIT}
\author{S.~Lockwitz} \affiliation{\FNAL}
\author{D.~Lorca} \affiliation{\Bern}
\author{W.~C.~Louis} \affiliation{\LANL}
\author{M.~Luethi} \affiliation{\Bern}
\author{B.~Lundberg}  \affiliation{\FNAL}
\author{X.~Luo} \affiliation{\Yale}
\author{A.~Marchionni} \affiliation{\FNAL}
\author{S.~Marcocci} \affiliation{\FNAL}
\author{C.~Mariani} \affiliation{\VTech}
\author{J.~Marshall} \affiliation{\Cambridge}
\author{J.~Martin-Albo} \affiliation{\Harvard}
\author{D.~A.~Martinez~Caicedo} \affiliation{\IIT}
\author{A.~Mastbaum} \affiliation{\Chicago}
\author{V.~Meddage} \affiliation{\KSU}
\author{T.~Mettler}  \affiliation{\Bern}
\author{G.~B.~Mills} \affiliation{\LANL}
\author{K.~Mistry} \affiliation{\Manchester}
\author{A.~Mogan} \affiliation{\Tennessee}
\author{J.~Moon} \affiliation{\MIT}
\author{M.~Mooney} \affiliation{\CSU}
\author{C.~D.~Moore} \affiliation{\FNAL}
\author{J.~Mousseau} \affiliation{\Michigan}
\author{M.~Murphy} \affiliation{\VTech}
\author{R.~Murrells} \affiliation{\Manchester}
\author{D.~Naples} \affiliation{\Pitt}
\author{P.~Nienaber} \affiliation{\StMarys}
\author{J.~Nowak} \affiliation{\Lancaster}
\author{O.~Palamara} \affiliation{\FNAL}
\author{V.~Pandey} \affiliation{\VTech}
\author{V.~Paolone} \affiliation{\Pitt}
\author{A.~Papadopoulou} \affiliation{\MIT}
\author{V.~Papavassiliou} \affiliation{\NMSU}
\author{S.~F.~Pate} \affiliation{\NMSU}
\author{Z.~Pavlovic} \affiliation{\FNAL}
\author{E.~Piasetzky} \affiliation{\TelAviv}
\author{D.~Porzio} \affiliation{\Manchester}
\author{G.~Pulliam} \affiliation{\Syracuse}
\author{X.~Qian} \affiliation{\BNL}
\author{J.~L.~Raaf} \affiliation{\FNAL}
\author{A.~Rafique} \affiliation{\KSU}
\author{L.~Rochester} \affiliation{\SLAC}
\author{M.~Ross-Lonergan} \affiliation{\Columbia}
\author{C.~Rudolf~von~Rohr} \affiliation{\Bern}
\author{B.~Russell} \affiliation{\Yale}
\author{D.~W.~Schmitz} \affiliation{\Chicago}
\author{A.~Schukraft} \affiliation{\FNAL}
\author{W.~Seligman} \affiliation{\Columbia}
\author{M.~H.~Shaevitz} \affiliation{\Columbia}
\author{R.~Sharankova} \affiliation{\Tufts}
\author{J.~Sinclair} \affiliation{\Bern}
\author{A.~Smith} \affiliation{\Cambridge}
\author{E.~L.~Snider} \affiliation{\FNAL}
\author{M.~Soderberg} \affiliation{\Syracuse}
\author{S.~S{\"o}ldner-Rembold} \affiliation{\Manchester}
\author{S.~R.~Soleti} \affiliation{\Oxford}\affiliation{\Harvard}
\author{P.~Spentzouris} \affiliation{\FNAL}
\author{J.~Spitz} \affiliation{\Michigan}
\author{J.~St.~John} \affiliation{\FNAL}
\author{T.~Strauss} \affiliation{\FNAL}
\author{K.~Sutton} \affiliation{\Columbia}
\author{S.~Sword-Fehlberg} \affiliation{\NMSU}
\author{A.~M.~Szelc} \affiliation{\Manchester}
\author{N.~Tagg} \affiliation{\Otterbein}
\author{W.~Tang} \affiliation{\Tennessee}
\author{K.~Terao} \affiliation{\SLAC}
\author{M.~Thomson} \affiliation{\Cambridge}
\author{R.~T.~Thornton} \affiliation{\LANL}
\author{M.~Toups} \affiliation{\FNAL}
\author{Y.-T.~Tsai} \affiliation{\SLAC}
\author{S.~Tufanli} \affiliation{\Yale}
\author{T.~Usher} \affiliation{\SLAC}
\author{W.~Van~De~Pontseele} \affiliation{\Oxford}\affiliation{\Harvard}
\author{R.~G.~Van~de~Water} \affiliation{\LANL}
\author{B.~Viren} \affiliation{\BNL}
\author{M.~Weber} \affiliation{\Bern}
\author{H.~Wei} \affiliation{\BNL}
\author{D.~A.~Wickremasinghe} \affiliation{\Pitt}
\author{K.~Wierman} \affiliation{\PNNL}
\author{Z.~Williams} \affiliation{\UTA}
\author{S.~Wolbers} \affiliation{\FNAL}
\author{T.~Wongjirad} \affiliation{\Tufts}
\author{K.~Woodruff} \affiliation{\NMSU}
\author{T.~Yang} \affiliation{\FNAL}
\author{G.~Yarbrough} \affiliation{\Tennessee}
\author{L.~E.~Yates} \affiliation{\MIT}
\author{G.~P.~Zeller} \affiliation{\FNAL}
\author{J.~Zennamo} \affiliation{\Chicago}\affiliation{\FNAL}
\author{C.~Zhang} \affiliation{\BNL}

\collaboration{The MicroBooNE Collaboration} \noaffiliation


